LumoTree: Path-Parallel Speculative Verification for Hybrid Language Models

Tree speculative decoding for recurrent-hybrid language models requires each accepted path to maintain consistent recurrent state, convolution history, and attention caches. We present LumoTree, a GPU serving design that coordinates verification and commitment through a shared tree descriptor. The verifier processes independent paths in parallel and reuses recurrent state tiles across local updates. Boundary states connect dependent paths. Accepted-path replay publishes the selected continuation into native running state, alongside coordinated convolution gathering and attention-cache remapping. Fused selection, device-resident acceptance, graph replay, and tree-aware attention integrate this organization into the serving cycle. The design separates temporary branch computation from persistent request state while retaining native prefix-cache interfaces. We evaluate numerical behavior, serving performance, and coding-agent outcomes on NVIDIA DGX Spark.

==> sections/native-continuation.tex <==
We examine native-reference reproducibility across independent processes as a prerequisite for full-model tree validation. Each condition covers 84 paths: a root-only continuation and 27 candidate paths for each of three calibration prefixes. Every path is repeated twice in each of two independent processes. The conditions distinguish natural prefill from an imported common starting state and separate target continuation from continuation coupled to the MTP drafter.

\begin{table}[t]
\caption{Cross-process native-reference agreement, in paths out of 84. State/logits requires identical published target state and full target logits. Joint choices requires the next target decision and the actual MTP spine and ordered top-three selections at every tested phase. A dash denotes an untested joint MTP condition.}
\label{tab:native-continuation}
\centering\footnotesize
\setlength{\tabcolsep}{3pt}
\begin{tabularx}{\columnwidth}{@{}Xrrr@{}}
\toprule
Starting-state control & Greedy & \shortstack{State/\\logits} & \shortstack{Joint\\choices} \\
\midrule
Natural prefill & 70/84 & 0/84 & -- \\
Common target state & 84/84 & 84/84 & -- \\
Common target and MTP state & 84/84 & 65/84 & 68/84 \\
\quad With fixed kernel selection & 84/84 & 65/84 & 68/84 \\
\bottomrule
\end{tabularx}
\end{table}

Natural-prefill continuation reproduces within each process but changes the greedy winner on fourteen paths across processes. The target-only control with common starting state reproduces identical target state, logits, and greedy decisions on all paths. When MTP continuation is included, greedy decisions remain stable on all paths, but target state and full logits agree on only 65, and joint target/draft choices on 68. Holding kernel selection fixed yields the same aggregate counts.

All sixteen paths with differing joint choices have long prefixes. Their within-process repetitions agree, and every principal MTP spine remains stable; the disagreements affect secondary top-three membership or order. The tested phases include initial MTP continuation, a follow-up, and continuation after consuming the pending target token. Common imported state and matched tokens and positions do not guarantee identical intermediate hidden tensors.

The sixteen joint-choice disagreements prevent this reference from supporting a full-model tree equivalence claim (Section~\ref{sec:limitations}).

